Collaborative Wideband Spectrum Sensing and Scheduling for Networked UAVs in UTM Systems

In this paper, we propose a data-driven framework for collaborative wideband spectrum sensing and scheduling for networked unmanned aerial vehicles (UAVs), which act as the secondary users to opportunistically utilize detected spectrum holes. To this end, we propose a multi-class classification problem for wideband spectrum sensing to detect vacant spectrum spots based on collected I/Q samples. To enhance the accuracy of the spectrum sensing module, the outputs from the multi-class classification by each individual UAV are fused at a server in the unmanned aircraft system traffic management (UTM) ecosystem. In the spectrum scheduling phase, we leverage reinforcement learning (RL) solutions to dynamically allocate the detected spectrum holes to the secondary users (i.e., UAVs). To evaluate the proposed methods, we establish a comprehensive simulation framework that generates a near-realistic synthetic dataset using MATLAB LTE toolbox by incorporating base-station~(BS) locations in a chosen area of interest, performing ray-tracing, and emulating the primary users channel usage in terms of I/Q samples. This evaluation methodology provides a flexible framework to generate large spectrum datasets that could be used for developing ML/AI-based spectrum management solutions for aerial devices.

==> figures/main_v1.tex <==
% % \documentclass[12pt, draftclsnofoot, onecolumn]{IEEEtran}

% \documentclass[conference,10pt]{IEEEtran}
% \usepackage[T1]{fontenc}



% \usepackage{amsmath,amssymb,amsmath,amsfonts}
% \usepackage{bm}
% \usepackage{bbm}
% \usepackage{graphicx}
% \usepackage[noadjust]{cite}
% \usepackage{citesort}
% \usepackage{epstopdf}

% \usepackage{algorithmic}
% \usepackage[ruled]{algorithm2e}
% \usepackage{url}
% \usepackage{makecell}
% \renewcommand{\algorithmicrequire}{\textbf{Input:}}
% \renewcommand{\algorithmicensure}{\textbf{Output:}}
% \usepackage{gensymb}
% \usepackage{color}
% \usepackage{lipsum}
% \usepackage{float}
% \usepackage{epstopdf}
% \usepackage[mathcal]{eucal}
% \usepackage{subfiles}
% \usepackage[T1]{fontenc}
% \usepackage{siunitx}
% % \usepackage{refcheck}
% \usepackage{tabulary}
% \usepackage{array}
% \usepackage{adjustbox}
% \usepackage[dvipsnames]{xcolor}
% \usepackage{times}
% \usepackage{placeins}
% \usepackage{textcomp}
% \usepackage[font=small]{caption}
% \usepackage{xcolor}
% \usepackage{tabularx}
% \usepackage{bm}
% \usepackage{enumerate}
% \usepackage{tikz}
% \usepackage{pgfplots}
% \usepackage{epstopdf}
% \usetikzlibrary{shapes,arrows}
% \usepackage[utf8]{inputenc}
% \usepackage{mathtools}
% \usepackage[utf8]{inputenc}
% \usepackage{xcolor}
% \usepackage{tikz}
% \usetikzlibrary{chains,arrows,calc,positioning}
% \pgfplotsset{compat=1.16}
% \definecolor{bittersweet}{rgb}{1.0, 0.44, 0.37}
% \definecolor{glaucous}{rgb}{0.38, 0.51, 0.71}
% \definecolor{gainsboro}{rgb}{0.86, 0.86, 0.86}
% \definecolor{babyblueeyes}{rgb}{0.63, 0.79, 0.95}
% \definecolor{silver}{rgb}{0.75, 0.75, 0.75}
% \definecolor{neoncarrot}{rgb}{1.0, 0.64, 0.26}
% \usepackage{soul}
% \usepackage{varwidth}
% % to split equations using dmath env
% \usepackage{breqn}
% % nice rules in tables
% \usepackage{booktabs}
% \usepackage{multirow}

% %%%%%%%%%%%%%%%%%%%%%%%%%%%
% \usepackage{enumitem}
% \usepackage{tabulary}
% \newcommand{\gio}[1]{\noindent \textcolor[rgb]{0.2,0.6,0.2} {{$\blacktriangleright$ 
%   {\textsf{[Gio]: #1}} $\blacktriangleleft$}}}
% \newcommand{\mynote}[1]{\noindent \textcolor{red} {{$\blacktriangleright$
%   \small{\textsf{#1}} $\blacktriangleleft$}}}
% \newcommand{\blue}[1]{\textcolor{blue}{#1}}
% \newcommand{\red}[1]{{\textcolor[rgb]{1,0,0}{#1}}}
% \newcommand{\green}[1]{{\textcolor[rgb]{0.2,0.6,0.2}{#1}}}
% \usepackage[normalem]{ulem}
% %%%%%%%%%%%%%%%%%%%%%%%%%%

% \input{acronyms.tex}

% \makeatletter

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%% LyX specific LaTeX commands.
% %% Because html converters don't know tabularnewline
% \providecommand{\tabularnewline}{\\}

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Textclass specific LaTeX commands.
%  % protect \markboth against an old bug reintroduced in babel >= 3.8g
%  \let\oldforeign@language\foreign@language
%  \DeclareRobustCommand{\foreign@language}[1]{%
%   \lowercase{\oldforeign@language{#1}}}

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%% User specified LaTeX commands.
% % for subfigures/subtables
% % \usepackage[caption=false,font=footnotesize]{subfig}
% \usepackage[font=small]{caption}%https://www.overleaf.com/project/5dea7e8d55668600017637bf
% % \usepackage[font=footnotesize]{subcaption}

% \usepackage{dblfloatfix}

% \input{commands.tex}

% \makeatother

% \IEEEoverridecommandlockouts

% \newcommand{\commentmh}[1]{{\emph{\textcolor{teal}{[MH: #1]}}}}

% \newcommand{\commentsr}[1]{{\emph{\textcolor{cyan}{[SR: #1]}}}}

% \newcommand{\norm}[1]{\left\lVert#1\right\rVert}


% \usepackage[top=0.705in, left=0.625in, bottom=1in, right=0.625in]{geometry}

% \begin{document}



% \title{{Spectrum Sharing for UAVs using multi-agent RL and deep neural networks}}



% % \author{
% % \IEEEauthorblockN{Sravan Reddy Chintareddy,   Morteza Hashemi}\\
% % \IEEEauthorblockA{Department of Electrical Engineering and Computer Science, University of Kansas}}
% % \thanks{The work of M. Mezzavilla and S. Rangan were supported by
% % NSF grants  1302336,  1564142,  1547332, and 1824434,  NIST, SRC, and the industrial affiliates of NYU WIRELESS.The work of Sravan R. Chintareddy and M. Hashemi were partially supported by the NSF grants CNS-1948511 and CNS-1955561.}}


% % make the title area
% \maketitle

% % As a general rule, do not put math, special symbols or citations
% % in the abstract or keywords.
% \begin{abstract}
% \input{abstract}
% \end{abstract}  


% % Note that keywords are not normally used for peer review papers.
% \begin{IEEEkeywords}
% Unmanned aerial vehicle (UAV).

% \end{IEEEkeywords}

% \IEEEpeerreviewmaketitle
% % \input{JournalExtension/Actionitems}

% \input{intro}

% % \input{background}
% %\input{raytracing.tex}
% \input{problem}

% % \input{derivations}
% \input{results}

% \input{conclusion}
% \pagebreak

% % Can use something like this to put references on a page
% % by themselves when using endfloat and the captionsoff option.
% %\ifCLASSOPTIONcaptionsoff
% %  \newpage
% %\fi
% % \nocite{*}
% \bibliographystyle{IEEEtran}
% \bibliography{bibl}

% \end{document}



